Keep It SimPool: Who Said Supervised Transformers Suffer from Attention Deficit?

Convolutional networks and vision transformers have different forms of pairwise interactions, pooling across layers and pooling at the end of the network. Does the latter really need to be different? As a by-product of pooling, vision transformers provide spatial attention for free, but this is most often of low quality unless self-supervised, which is not well studied. Is supervision really the problem? In this work, we develop a generic pooling framework and then we formulate a number of existing methods as instantiations. By discussing the properties of each group of methods, we derive SimPool, a simple attention-based pooling mechanism as a replacement of the default one for both convolutional and transformer encoders. We find that, whether supervised or self-supervised, this improves performance on pre-training and downstream tasks and provides attention maps delineating object boundaries in all cases. One could thus call SimPool universal. To our knowledge, we are the first to obtain attention maps in supervised transformers of at least as good quality as self-supervised, without explicit losses or modifying the architecture. Code at: https://github.com/billpsomas/simpool.

==> app/exp-training.tex <==
\subsection{Training}
\label{sec:more-train}

%------------------------------------------------------------------------------
\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
	font=\scriptsize,
	width=1.05\linewidth,
	height=0.6\linewidth,
	xlabel={epochs},
	ylabel={accuracy},
	ymin=65,
	legend pos=south east,
]
\pgfplotstableread{
	 ep  cls   our
	  0  63.6  64.7
	 10  70.4  71.6
	 20  70.9  72.2
	 30  71.1  72.4
	 40  71.3  72.6
	 50  71.4  72.7
	 60  71.4  72.7
	 70  71.5  72.7
	 80  71.5  72.8
	 90  71.5  72.8
	100  71.5  72.8
}{\train}
\addplot[smooth,blue] table[x=ep,y=cls] {\train}; \leg{Baseline (\cls)}
\addplot[smooth,red] table[x=ep,y=our] {\train}; \leg{\ours}
\end{axis}
\end{tikzpicture}
\caption{Image classification top-1 accuracy (\%) \vs training epochs; linear probing on ImageNet-1k. Self-supervised pre-training with DINO~\cite{dino}.}
\label{fig:SelfProbe}
\end{figure}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
	font=\scriptsize,
	width=1.05\linewidth,
	height=0.6\linewidth,
	xlabel={epochs},
	ylabel={accuracy},
	ymin=40,
	legend pos=south east,
]
\pgfplotstableread{
	 ep  ViT-S   ViT-S+\ours
	  0  0.1  0.1
	 10  4.0  4.0
	 20  36.4  39.9
	 30  49.6  55.2
	 40  61.0  64.3
	 50  65.5  68.6
	 60  68.1  70.7
	 70  69.9  72.1
	 80  71.4  73.1
	 90  72.3  74.0
	100  72.7  74.3
}{\train}
\addplot[smooth,blue] table[x=ep,y=ViT-S] {\train}; \leg{ViT-S}
\addplot[smooth,red] table[x=ep,y=ViT-S+\ours] {\train}; \leg{ViT-S+\ours}
\end{axis}
\end{tikzpicture}
\caption{Image classification top-1 accuracy (\%) \vs training epochs on ImageNet-1k. Supervised training on ViT-S.}
\label{fig:accvsepochsVIT}
\end{figure}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
	font=\scriptsize,
	width=1.05\linewidth,
	height=0.6\linewidth,
	xlabel={epochs},
	ylabel={accuracy},
	ymin=59,
	legend pos=south east,
]
\pgfplotstableread{
	 ep  ResNet-50   ResNet-50+\ours
	  0  0.1  0.1
	 10  56.0  58.9
	 20  63.4  65.6
	 30  66.4  68.7
	 40  68.9  70.7
	 50  70.7  72.2
	 60  72.3  73.7
	 70  73.7  74.6
	 80  75.7  76.3
	 90  77.0  77.6
	100  77.4  78.0
}{\train}
\addplot[smooth,blue] table[x=ep,y=ResNet-50] {\train}; \leg{ResNet-50}
\addplot[smooth,red] table[x=ep,y=ResNet-50+\ours] {\train}; \leg{ResNet-50+\ours}
\end{axis}
\end{tikzpicture}
\caption{Image classification top-1 accuracy (\%) \vs training epochs on ImageNet-1k. Supervised training on ResNet-50.}
\label{fig:accvsepochsRESNET}
\end{figure}
%-------------

%------------------------------------------------------------------------------
\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
	font=\scriptsize,
	width=1.05\linewidth,
	height=0.6\linewidth,
	xlabel={epochs},
	ylabel={k-NN},
	ymin=59,
	legend pos=south east,
]
\pgfplotstableread{
	 ep ViT-S   ViT-S+\ours
	  0  1.0  2.8
	 15  49.2  51.0 % 51.0 approximately interpolate
	 30  60.0  61.7
	 45  62.9  63.5 % 63.5 approximately interpolate
	 60  64.8  66.0
	 75  67.1  68.0 % 68.0 approximately interpolate
	 90  68.6  69.4
	100  68.7  69.6
}{\train}
\addplot[smooth,blue] table[x=ep,y=ViT-S] {\train}; \leg{ViT-S}
\addplot[smooth,red] table[x=ep,y=ViT-S+\ours] {\train}; \leg{ViT-S+\ours}
\end{axis}
\end{tikzpicture}
\caption{Image classification top-1 accuracy (\%) \vs training epochs on ImageNet-1k. Supervised training on ViT-S.}
\label{fig:knnvsepochsVIT}
\end{figure}
%-------------

\paragraph{Image classification}

\autoref{fig:SelfProbe} shows that \Ours outperforms the default \cls at 90\% fewer training epochs. \iavrc{Say more.}



==> app/main.tex <==
\title{Keep it \Ours: Who said supervised transformers suffer from attention deficit? \\ {\emph{Supplementary material}}}
\renewcommand{\teaser}{}
\maketitle

\setcounter{page}{1}
\iccvrulercount=1

\appendix


==> tex/algorithm-1.tex <==
\begin{algorithm}
\caption{\ours pseudocode}\label{alg:simpool}
\begin{algorithmic}
\Require $\vX \in \real^{d \times p}$

\State $\vu^0~\gets X \vone_p / p$

\State $\vX~~\gets layer\_norm(\vX)$

\State $\vq~~~\gets \lrn{W_Q}\vu^0 $

\State $\vK~~\gets \lrn{W_K}\vX $

\State $\va~~~\gets \vsigma_2 \left( \vK\tran \vq / \sqrt{d} \right)$

\State $\vu~~~\gets ((\vX - \min \vX)^{\alpha} \va )^{1/\alpha}$

\State \Return $\vu$
\end{algorithmic}
\end{algorithm}

==> tex/bboxes.tex <==
\small
\centering
\setlength{\tabcolsep}{1.14pt}
\begin{tabular}{cccccccc}
	\fig[.48]{bboxes/ship_original.pdf}                 &
	\fig[.48]{bboxes/ship_random_30.pdf}                \\

	\fig[.48]{bboxes/ship_original.pdf}                 &
	\fig[.48]{bboxes/ship_random_30.pdf}                \\

%	(a) Input                                                &
%	(b) Random                                               &
%	(c) Random                                               &
%	(d) Block                                                &
%	(e) Attention                                            &
%	(f) \ours                                                \\

%	Image                                                    &
%	(30)                                                     &
%	(75)                                                     &
%	Wise                                                     &
%	Map                                                      &
%	High                                                     \\
\end{tabular}


==> tex/exp-ablation-1.tex <==
\subsection{Ablation Study}
\label{sec:ablation}

% %------------------------------------------------------------------------------
% \begin{table*}[t]
% \small
% \centering
% \setlength{\tabcolsep}{1pt}
% \caption{\emph{The effect of $\alpha$ on attention maps}: ResNet-18 on Imagenet $20\%$.}
% \label{tab:r18alpha}
% \begin{tabular}{lcccccccc}
%     {}                                                    &
% 	\fig[.1]{background_shark/only_fg.pdf}              &
% 	\fig[.1]{background_shark/mixed_same.pdf}           &
% 	\fig[.1]{background_shark/mixed_rand.pdf}           &
% 	\fig[.1]{background_shark/mixed_next.pdf}           &
% 	\fig[.1]{background_shark/no_fg.pdf}                &
% 	\fig[.1]{background_shark/only_bg_b.pdf}             &
% 	\fig[.1]{background_shark/only_bg_t.pdf}             &
% 	\fig[.1]{background_shark/original.pdf}             \\
%
% \toprule
% \mr{2}{\Th{Model}} & \mc{7}{\Th{$\alpha$}} \\ \cmidrule{2-9}
%             & official & 0.5 & 1.0 & 1.5  & 2.0  & 2.5  & 3.0  & 5.0 \\ \midrule
% ResNet-18  &  54.9    & 55.7   & 56.6 & 56.9 & \bf{57.1} & 56.8 & 56.6 & 54.5 \\
% \bottomrule
% \end{tabular}
% \end{table*}
% %------------------------------------------------------------------------------




%------------------------------------------------------------------------------
%\begin{figure}
%\centering
%\begin{tikzpicture}
%\begin{axis}[
%	title={},
%	xlabel={$\alpha$},
%	ylabel={$Accuracy$},
%	width=7cm, height=5cm,
%	xmin=0.5, xmax=5.0,
%	ymin=55.0, ymax=65.0,
%	legend pos=south east,
%	legend columns=1,
%	ymajorgrids=true,
%	grid,
%]
%	\addplot[red,mark=*]coordinates {
%		(0.50, 55.9)(1.0,56.6)(1.25, 56.6)(1.5, 57.0)(2.0, 57.1)(2.5, 56.8)(3.0, 56.6)(5.0, 56.2)
%		}; \leg{ResNet-18}
%	\addplot[blue,mark=*]coordinates {
%		(0.50, 63.0)(0.75, 63.4)(1.0,63.8)(1.25, 64.2)(1.5, 64.1)(2.0, 64.1)(2.5, 63.9)(3.0, 63.7)(5.0, 63.5)
%		}; \leg{ViT-T}
%\end{axis}
%\end{tikzpicture}
%\vspace{-6pt}
%\caption{.}
%\label{fig:alphas-plot}
%\end{figure}
%------------------------------------------------------------------------------


%------------------------------------------------------------------------------
\begin{table}[t]
\small
\begin{center}
\setlength{\tabcolsep}{1pt}

\begin{tabular}{lcc|ccccccc} 
\mc{3}{(a)} & \mc{6}{(b)}  \\ \toprule
\Th{Ablation on} & \Th{Options} & \Th{Acc.} & \mc{3}{\Th{Linears}} &  \mc{3}{\Th{LNs}} & \Th{Acc.}  \\ \midrule
\mr{2}{$A$} & $\vsigma_2(S_i/\sqrt{d})_{i=1}^m$ & 56.6 & $q$    & $k$        & $v$   & $q$    & $k$ & $v$   &    \\ \cmidrule{4-9}
 & $\norm{\exp{S_i}}_{L_{2}}$ & 55.5 &\checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \bf{57.0}  \\\midrule
\mr{2}{\red{\Th{Layers}}}   & 3 & 56.8 & \gp{\checkmark} & \gp{\checkmark} &  & \checkmark & \checkmark & \checkmark & \bf{56.6}  \\
  & 5 & 56.9 & \checkmark &  &  & \checkmark & \checkmark & \checkmark & 56.5  \\\cmidrule{1-3}
 \mr{2}{\Th{Iter}}     & 3 & 56.5 &   & \checkmark &  & \checkmark & \checkmark & \checkmark & 56.4  \\
   & 5 & 56.4 & &  &  & \checkmark & \checkmark & \checkmark & 55.6  \\ \midrule
\mr{2}{$U^0$} & $\gp{U}$ & 56.3 & \checkmark & \checkmark &  & \checkmark & \checkmark &  & 56.3  \\
 & $\|X\|$ & 56.5 & \checkmark & \checkmark &  & \checkmark &  &  & 56.3  \\\cmidrule{1-3}
\mr{2}{$s(\vx, \vy)$} & $-\|\vx-\vy\|^2$ & 56.4 & \checkmark & \checkmark &  &  & \checkmark &  & 56.1  \\
  & $cosine$ & 56.3 & \checkmark & \checkmark &  &  & \gp{\checkmark} & \gp{\checkmark} & \bf{56.6}  \\ \cmidrule{1-3}
\mr{2}{$\hp{k}$ - max} & 2 & 56.5 & \checkmark & \checkmark &  &  &  & \checkmark & 56.4  \\
 & 5 & 56.4 & \checkmark & \checkmark &  & \checkmark &  & \checkmark & 56.2 \\ \cmidrule{4-10}
\mr{2}{$\hp{k}$ - concat + proj}  & 2 & 56.5 & &  &  &  &  \gp{\checkmark} &  \gp{\checkmark} & 56.2  \\
  & 5 & 55.9 & \gp{\checkmark} & \gp{\checkmark} &  &  &  &  & \red{54.4}  \\ \cmidrule{1-3}
$\phi_Q(\vU)$, $\phi_K(\vX)$ & $\gp{W_Q}=\gp{W_K}$ & 56.4 & &  &  &  &  &  & 54.5  \\ \midrule
 \Ours  &  & \bf{57.1} & \mc{6}{\Th{GAP}}  & 54.9  \\ \bottomrule
\end{tabular}
\end{center}
\caption{\Ours ablation on \imagenet 20\% using ResNet-18 trained for 100 epochs. On (a) ablation of different components and on (b) Linears and LayerNorms.}
\label{tab:ablationall}
\end{table}
%------------------------------------------------------------------------------



%------------------------------------------------------------------------------
%\begin{table}[t]
%\small
%\centering
%\setlength{\tabcolsep}{2.5pt}
%\caption{\Ours ablation on \imagenet 20\% using ResNet-18.}
%\label{tab:ablation1}
%\begin{tabular}{lcccc} \toprule
%\Th{Ablation on} & \Th{Options} & \Th{Accuracy} & \Th{Parameters}\\ \midrule

% \mr{2}{$A$} & $\vsigma_2(S_i/\sqrt{d})_{i=1}^m$ & 56.6 & &\\ 
% & $\norm{\exp{S_i}}_{L_{2}}$ & 55.5 & &\\ \midrule
%\mr{2}{\red{\Th{Layers}}}   & 3 & 56.8 & &\\
%                       & 5 & 56.9 & &\\ \midrule
% \mr{2}{\Th{Iter}}     & 3 & 56.5 & &\\
%                      & 5 & 56.4 & &\\ \midrule
%\mr{2}{$U^0$} & $\gp{U}$ & 56.3 & &\\
%                  & $\|X\|$ & 56.5 & &\\ \midrule
%\mr{2}{$s(\vx, \vy)$} & $-\|\vx-\vy\|^2$ & 56.4 & &\\
%                  & $cosine$ & 56.3 & &\\ \midrule
%\mr{2}{$\hp{k}$ - max} & 2 & 56.5 & &\\
%                  & 5 & 56.4 & &\\ \midrule
%\mr{2}{$\hp{k}$ - concat + proj}  & 2 & 56.5 & &\\
%                  & 5 & 55.9 & &\\
%\midrule
%$\phi_Q(\vU)$, $\phi_K(\vX)$ & $\gp{W_Q}=\gp{W_K}$ & 56.4 & &\\ \midrule
%\Ours  &  & \bf{57.1} & &\\
%\bottomrule
%\end{tabular}
%\end{table}
%------------------------------------------------------------------------------


%------------------------------------------------------------------------------
%\begin{table}[t]
%\small
%\centering
%\setlength{\tabcolsep}{3pt}
%\caption{Linears and LayerNorms. ResNet-18 trained on ImageNet 20\% for 100 epochs.}
%\label{tab:linearslayernorms2}
%\begin{tabular}{cccccccc} \toprule
%\mc{3}{\Th{Linears}} &  \mc{3}{\Th{LNs}} & \mr{2}{\Th{Accuracy}} & \mr{2}{\Th{MaxBoxAccV2}} \\ \cmidrule{1-6}
%$q$    & $k$        & $v$   & $q$    & $k$ & $v$   & &    \\ \midrule
%\checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \bf{57.0} & 52.56 \\\midrule
%\gp{\checkmark} & \gp{\checkmark} &  & \checkmark & \checkmark & \checkmark & \bf{56.6} & 54.36 \\
%\checkmark &  &  & \checkmark & \checkmark & \checkmark & 56.5 & \bf{54.64} \\
%  & \checkmark &  & \checkmark & \checkmark & \checkmark & 56.4 & - \\
%  &  &  & \checkmark & \checkmark & \checkmark & 55.6 & - \\ \midrule
%\checkmark & \checkmark &  & \checkmark & \checkmark &  & 56.3 & - \\
%\checkmark & \checkmark &  & \checkmark &  &  & 56.3 & - \\
%\checkmark & \checkmark &  &  & \checkmark &  & 56.1 & - \\
%\checkmark & \checkmark &  &  & \gp{\checkmark} & \gp{\checkmark} & \bf{56.6} & \bf{53.76} \\
%\checkmark & \checkmark &  &  &  & \checkmark & 56.4 & - \\
%\checkmark & \checkmark &  & \checkmark &  & \checkmark & 56.2 & - \\\midrule
% &  &  &  &  \gp{\checkmark} &  \gp{\checkmark} & 56.2 & - \\
%\gp{\checkmark} & \gp{\checkmark} &  &  &  &  & \red{54.4} & - \\
% &  &  &  &  &  & 54.5 & - \\ \midrule
%  \mc{6}{\Th{GAP}}  & 54.9 & - \\ \bottomrule
%\end{tabular}
%\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
%\begin{table}[t]
%\small
%\centering
%\setlength{\tabcolsep}{3pt}
%\caption{Trained on \gkakoc{maybe rerun on 100\%} \red{20\%} of the ImageNet for 100 epochs. (ResNet-18 contains 11.2M parameters)}
%\label{tab:table_name3}
%\begin{tabular}{lccccccc} \toprule
%\mr{2}{\Th{Models}} & \mc{6}{\Th{Alpha}} \\ \cmidrule{2-8}
%           & official    & 1.0        & 1.25   & 1.5    & 2.0 & 2.5      & 3.0   \\ \midrule
%ResNet-18 & 54.9         & 56.6       & 56.5       & 56.9    & 57.1    & 56.8        & - \\ \bottomrule
%\end{tabular}
%\end{table}
%------------------------------------------------------------------------------

\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
	title={},
	xlabel={$\alpha$},
	ylabel={$Accuracy$},
	width=7cm, height=5cm,
	xmin=0.5, xmax=5.0,
	ymin=54.0, ymax=58.0,
	legend pos=south east,
	legend columns=1,
	ymajorgrids=true,
	grid,
]
	\addplot[red,mark=*]coordinates {
		(0.50, 55.9)(1.0,56.6)(1.5, 56.9)(2.0, 57.1)(2.5, 56.8)(3.0, 56.6)(5.0, 54.5)
		}; \leg{ResNet-18}
\end{axis}
\end{tikzpicture}
\vspace{-6pt}
\caption{.}
\label{fig:alphas-plot}
\end{figure}



We perform an ablation study to analyze the different choices forming \Ours. We conduct these experiments using ResNet-18 supervised trained on 20\% of the ImageNet-1k. In \autoref{tab:ablationall} \red{(a)}, we examine different pooling strategies complementary to \autoref{fig:tourn}. In \autoref{tab:ablationall} \red{(b)}, we ablate the linear layers and layer normalizations. In \autoref{fig:alphas-plot}, we examine the $\alpha$ hyperparameter.

\paragraph{Ablation of design}

We analyze the performance of \Ours by ablating the main choices. In \autoref{tab:ablationall} \red{(a)}, we ablate the attention function $A$, the number of iterations with (\Th{Layers}) or without (\Th{Iter}) shared parameters across the steps, the initialization $U^0$ of the pooling, the pairwise similarities $s(\vx, \vy)$, as well as the number $\hp{k}$ of pooled representations and their final aggregation, i.e., maximum across the output logits or concatenation and projection to a final representation. Moreover, we examine a simpler approach with only one shared linear layer on the queries and keys, i.e., $\gp{W_Q}=\gp{W_K}$. We observe that ..\gkako{TODO}..

\paragraph{Ablation of linear and normalization}

In \autoref{tab:ablationall} \red{(b)}, we systematically ablate the different linear and normalization layers frequently appearing in attention modules. We aim to gain insights into the contributions of each component to the overall performance of \Ours and identify the most critical factors for achieving simplicity and satisfactory accuracy. We show that ..\gkako{TODO}.. 

Exploiting linear layers and layer normalization for all three $q, k, v$ slightly increase the classification accuracy. However, we highlight that this setup achieves a 52.56 MaxBoxAccV2 score compared to the \Ours strategy, which achieves 53.76. This is a testament to \Ours's accurate localization properties.

\paragraph{Ablation of alpha}

In \autoref{fig:alphas-plot}, we observe that ..\gkako{TODO}..


\gkakoc{Will we show these 1. "show property of k-means 2 (bg-fg). show iterations?" and 2. "show respective attention maps"?}


%\newcommand*\rot{\rotatebox{40}}

%\begin{table}[t]
%\small
%%\scriptsize
%\centering
%\setlength{\tabcolsep}{1.5pt}
%\caption{Linears and LayerNorms. ResNet-18 trained on ImageNet 20\% for 100 epochs.}
%\label{tab:linearslayernorms2}
%\begin{NiceTabular}%{l|c|c|c@{\hspace{-1ex}}c@{\hspace{-1ex}}c@{\hspace{-1ex}}c|c@{\hspace{-1ex}}c@{\hspace{-1ex}}c@{\hspace{-1ex}}c@{\hspace{-1ex}}c@{\hspace{-1%ex}}c|c@{\hspace{-1ex}}c@{\hspace{-1ex}}c@{\hspace{-1ex}}c}
%\Hline
%\Block{3-1}{\Th{LNs}} & q & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  & \checkmark & % &  &   \\
%%& k & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & \gp{\checkmark} & &  & \gp{\checkmark} & % &   \\
%
%& v & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  & \gp{\checkmark} & \checkmark & \checkmark & \gp{\checkmark} %&  &   \\
%\midrule
%
%
%\Block{3-1}{\Th{Linears}} & q & \checkmark & \gp{\checkmark} & \checkmark &  &  & \checkmark & \checkmark & \checkmark & \checkmark & %\checkmark & \checkmark &  & \gp{\checkmark} &   \\
%                          &  k & \checkmark & \gp{\checkmark} &  & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \gp{\checkmark} &   \\
%                          & v & \checkmark &  &  &  &  & &  &  &  &  &  &  &  &   \\
%\midrule
%
%\Block{1-2}{\Th{Accuracy}} & & \rot{\bf{57.0}} & \rot{\bf{56.6}}  & \rot{56.5} & \rot{56.4} & \rot{55.6} & \rot{56.3} & \rot{56.3} & %\rot{56.1} & \rot{\bf{56.6}} & \rot{56.4} & \rot{56.2} & \rot{56.2} & \rot{54.4} & \rot{54.5} \\
%\bottomrule
%
%\end{NiceTabular}
%
%\end{table}

==> tex/exp-analysis-1.tex <==
\subsection{Experimental Analysis}
\label{sec:analysis}

%------------------------------------------------------------------------------
\begin{figure}[htbp]
\centering
\begin{tikzpicture}[
	group/.style={draw,fill=white,fill opacity=.8},
]
    \begin{axis}[
        x tick label style={rotate=45,anchor=east},
        enlarge x limits=0.05,
        ymin=52,
        ymax=57.5,
        ybar,
        legend style={at={(0.5,-0.10)},anchor=north},
        xtick={0, 1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13},
        xticklabels={GAP \cite{resnet},max \cite{mac},GAP+max \cite{gapmax},GeM \cite{gem},LSE \cite{lse},HOW \cite{how},OTK \cite{otk},Slot \cite{slot},SE \cite{se},CBAM \cite{cbam},Gather-Excite \cite{gatherexcite},ViT \cite{vit},Cait \cite{cait},SimPool},
        width={0.52\textwidth},
        height={0.42\textwidth},
        nodes near coords,
        nodes near coords align={vertical},
        ]
        
        \addplot coordinates {
            (0, 54.9)
            (1, 54.0)
            (2, 54.6)
            (3, 54.2) 
            (4, 55.3) 
            (5, 54.8) 
            (6, 55.8) 
            (7, 56.6) 
            (8, 55.7) 
            (9, 55.6) 
            (10, 55.9) 
            (11, 56.1) 
            (12, 56.6)
            (13, 57.1)
            %(GeM\cite{gem},54.2)
            %(LSE\cite{lse},55.3)
            %(HOW\cite{how},54.8)
            %(OTK\cite{otk},55.8)
            %(Slot\cite{slot},56.6)
            %(SE\cite{se},55.7)
            %(CBAM\cite{cbam},55.6)
            %(Gather-Excite\cite{gatherexcite},55.9)
            %(ViT\cite{vit},56.1)
            %(Cait\cite{cait},56.6)
            %(SimPool,57.1)
        };
        \node[group,minimum width=88] at (axis cs:2.5, 52.5) {G1};
        \node[group,minimum width=28] at (axis cs:6.5, 52.5) {G2};
        \node[group,minimum width=42] at (axis cs:9,   52.5) {G3};
        \node[group,minimum width=28] at (axis cs:11.5,52.5) {G4};
    \end{axis}
\end{tikzpicture}
\caption{\emph{Image classification} (top-1 accuracy, \%) on the 20\% of ImageNet-1k. Supervised training of ResNet-18 for 100 epochs. SimPool outperforms all the other pooling methods.}
\label{fig:poolcompetition}
\end{figure}

Following \autoref{tab:land}, we reproduce the landscape of pooling methods creating a \KK{[pooling]} tournament \KK{[remove:]}of pooling methods \KK{[add fig ref here:]}(\autoref{fig:poolcompetition}). We train ResNet-18 on 20\% of ImageNet-1k for 100 epochs.  The goal of this analysis is the experimental study of different pooling methods - without necessarily having been defined as such - under equal terms proposed for (a) different tasks, e.g. instance-level or category-level, (b) used with different networks, e.g. convolutional networks or vision transformers, (c) having different properties and different use. More analysis is given in the Supplementary.

\emph{Group 1} mainly consists of parameter-free like GAP \cite{nin}, max \cite{mac}, GAP + max \cite{gapmax} or attention-free like GeM \cite{gem} and LSE \cite{lse}  methods. HOW \cite{how} is the only method to use attention (parameter-free), but this is not reflected in its performance (as a boost). LSE is performing the best, while GAP is the one following. In general, we observe that the 'simple' methods of this group seem to perform relatively poor comparing with the more complex methods of the other groups. 

\bill{\emph{Group 2} incorporates methods with $k > 1$. For OTK \cite{otk} we ... . Slot \cite{slot} is not originally introduced neither as a pooling operation nor for image classification. Thus, we define and experiment with three different setups, i.e. (number of slots, iters) = $(3,1), (3,3), (5,3)$. We report here results of the best setup, i.e. $(3,3)$. To obtain only one final representation, we take the max over the channels of the three vectors.}

\emph{Group 3} refers to parametric attention-based methods, i.e. methods that aim to improve the performance of the model by adaptively weighting features based on their importance for the task. While initially proposed as modules within the architecture, rather than simple pooling operations, we adapt them to our tournament by performing a global average pooling at the end. As an extension of SE, Gather-Excite performs the best.

\emph{Group 4} refers to more recent parametric attention-based methods proposed in vision transformers. ViT \cite{vit} refers to the well-known multi-head scaled dot product self-attention, which is incorporated as a single module at the end of the model. The CLS is parametric and we use four heads. Cait \cite{cait} is the same operation with the only difference that the patch embeddings are fixed and iterations exist. The CLS is again parametric. We use four heads, we incorporate a single Cait module at the end of the model and we set iterations \bill{=1}. In this group, Cait performs the best. 

Having a simple design and adopting the appropriate components from each method, SimPool, outperforms all the other methods.

Following the results of the tournament, we distinguish the best performing method of each group and qualify it for \autoref{sec:bench}, i.e. experiments on the 100\% of ImageNet-1k.

%------------------------------------------------------------------------------
%\begin{table}[t]
%\small
%\centering
%\setlength{\tabcolsep}{2.5pt}
%\caption{Classification accuracy on Imagenet 20\% using ResNet-18 and ViT-T with different pooling strategies.}
%\label{tab:table_name}
%\begin{tabular}{lccc} \toprule
%\Th{Method} & \Th{ResNet-18} & \Th{ViT-T} & \\ \midrule
% GAP \cite{resnet} & 54.9 & - & \\
%max \cite{mac} & 54.0 & - & \\
%GAP + max & 54.6 & - & \\
%GeM \cite{gem} & 54.0 & - & \\
%LSE \cite{lse} & 55.3 & - & \\
%HOW \cite{how} & 54.4 & - & \\ \midrule
%OTK \cite{otk} & 55.8 & - & \\
%Slot \cite{slot} & - & - & \\ \midrule
%SE \cite{se} & - & - & \\
%CBAM \cite{cbam} & 55.6 & - & \\
%Gather-Excite \cite{gatherexcite} & 55.9 & - & \\ \midrule
%ViT \cite{vit} & - & - & \\
%Cait \cite{cait} & 56.6 & - & \\ \midrule
%\ours & \bf{57.1} & - & \\
%\bottomrule
%\end{tabular}
%\end{table}
%------------------------------------------------------------------------------



%- Other pooling strategies: R-18 on Imagenet 20\% subset
%are we going to categorize them somehow?
%------------------------------------------------------------------------------


%------------------------------------------------------------------------------
%\begin{table}[t]
%\small
%\centering
%\setlength{\tabcolsep}{1pt}
%\caption{CorLoc for object discovery using \gkako{LOST}~\cite{lost} on \gkako{ResNet-50} backbones pretrained on ImageNet-1k with \gkako{DINO} for 100 epochs.}
%\label{tab:corloc_lost_Resnet}
%\begin{tabular}{lccc} \toprule
%\Th{Method} & \Th{VOC07} & \Th{VOC12} & \Th{COCO} \\ \midrule
%Default & 40.33 & 46.25 & 30.70   \\
%Ours & \bf{-} & \bf{-} & \bf{-}  \\
%\bottomrule
%\end{tabular}
%\end{table}
%-----------

%------------------------------------------------------------------------------
%\begin{table}[t]
%\small
%\centering
%\setlength{\tabcolsep}{1pt}
%\caption{CorLoc for object discovery using \gkako{LOST}~\cite{lost} on \gkako{ConvNeXt} backbones \gkako{supervised} pretrained on ImageNet-1k for 100 epochs.\gkakoc{HERE WE USED THE K OF CROSSATT INSTEAD OF RAW FEATURES}}
%\label{tab:corloc_lost_convnext}
%\begin{tabular}{lccc} \toprule
%\Th{Method} & \Th{VOC07} & \Th{VOC12} & \Th{COCO} \\ \midrule
%Default & 31.31 & 36.44 & 23.98   \\
%Ours & \bf{39.31} & \bf{44.64} & \bf{27.11}  \\
%\bottomrule
%\end{tabular}
%\end{table}
%-----------

%------------------------------------------------------------------------------
%\begin{table}[t]
%\small
%\centering
%\setlength{\tabcolsep}{1pt}
%\caption{CorLoc for object discovery using \gkako{DINO-seg}~\cite{lost} on \gkako{ViT-S} backbones \gkako{supervised} pretrained on ImageNet-1k for 100 epochs.}
%\label{tab:corloc_dinoseg_vit}
%\begin{tabular}{lccc} \toprule
%\Th{Method} & \Th{VOC07} & \Th{VOC12} & \Th{COCO} \\ \midrule
%Default & 11.14 & 9.97 & 14.34   \\
%Ours & \bf{40.63} & \bf{40.46} & \bf{37.97}  \\
%\bottomrule
%\end{tabular}
%\end{table}
%-----------



%------------------------------------------------------------------------------
%\begin{table}[t]
%\small
%\centering
%\setlength{\tabcolsep}{3pt}
%\caption{\emph{video object segmentation} (mean region similarity $\cJ_m$ and contour-based accuracy $\cF_m$, \%) on DAVIS 2017~\cite{davis}, without fine-tuning. Models pre-trained on 100\% ImageNet-1k training set for 100 epochs.}
%\label{tab:100percDownStreamVid}
%\begin{tabular}{lccc} \toprule
%\mr{2}{\Th{Method}} & \mc{3}{DAVIS 2017}                     \\ \cmidrule{2-4}
%                    & $(\cJ\&\cF)_m$ & $\cJ_m$   & $\cF_m$   \\ \midrule
%ViT-S                & \bf{61.4}           & \bf{59.6}      & \bf{63.2}      \\
%ViT-S + SimPool          & 60.3  & 58.3  & 62.3     \\
%\bottomrule
%\end{tabular}
%\end{table}
%------------------------------------------------------------------------------



==> tex/exp-bench-1.tex <==
\subsection{Benchmark}
\label{sec:bench}

%------------------------------------------------------------------------------
%\begin{table*}[ht]
%\small
%\centering
%\setlength{\tabcolsep}{3pt}
%\caption{Top-1 accuracy on ImageNet validation set. (a) Supervised classification results; (b) Self-supervised %DINO pre-training results measured by k-NN. All models are trained on 100\% ImageNet-1k for 100 epochs.}
%\label{tab:100percImageNet}
%\begin{tabular}{lccccc|ccccc} \toprule
%\mr{2}{\Th{Architecture}} & \mc{5}{(a) \Th{Supervised}} & \mc{5}{(b) \Th{Self-supervised}} \\  \cmidrule{2-11} 
% &  \Th{Default} & \Th{COMP1} & \Th{COMP2} & \Th{GAP-CLS} & \Th{GEM} & \Th{Default} & \Th{COMP1} & \Th{COMP2} & %\Th{GAP-CLS} & \Th{GEM} \\
%\midrule
%ResNet-50    &  77.4     & -& - & needed?   &  78.0   & 62.2  & - & - &  63.9 &  \emph{running}  \\
%ConvNeXt-S    &  81.1   & - & - &  81.5 & 81.7  & \emph{running}  & - & - &  \blue{62.3}  &  - \\
%ViT-S    &  72.7  & - & - &  74.3   & \red{74.2}  &    68.9    & - & - & 69.8  & \red{69.7}  \\
%\bottomrule
%\end{tabular}
%\end{table*}
%------------------------------------------------------------------------------

%We train \resnet50, \convnext and  \vits on \imagenet for 100 epochs using 


\paragraph{Image Classification} In \autoref{tab:Super100percImageNet}, we train ResNet-50, ConvNeXt-S and ViT-S on the 100\% of ImageNet-1k for 100 epochs. We employ Cait, Slot and Gather-Excite \emph{i.e.,} the best performing methods of the \KK{[pooling]} tournament \KK{[remove:]}of pooling methods. We follow exactly the same setup as previous. 

SimPool outperforms all the methods, improving the baseline by 0.6\% using convolutional networks and by 1.6\% using vision transformer, showing some early signs of consistency across different networks. Gather-Excite performs well when integrated to convolutional networks, \emph{i.e.,} improves baseline by 0.2\%, but performs poor with vision transformer. \bill{Slot... Cait  kk:why 77.3 red? ... }

\begin{table}[ht]
\small
\centering
\setlength{\tabcolsep}{3pt}
\caption{\emph{Image classification} (top-1 accuracy, \%) on the 100\% of ImageNet-1k. Supervised training of ResNet-50, ConvNeXt-S and ViT-S for 100 epochs.}
\label{tab:Super100percImageNet}
\begin{tabular}{lccc} 
\toprule
\mr{2}{\Th{Method}} & \mc{3}{\Th{Architecture}} \\  \cmidrule{2-4} 
 & \Th{ResNet-50} & \Th{ConvNeXt-S} & \Th{ViT-S} \\
\midrule
Default    &  77.4   & 81.1   & 72.7 \\
+ Cait \cite{cait}    &  \red{77.3}   & \emph{running}   & \red{72.6} \\
+ Slot \cite{slot}    & 77.3   & \emph{running}   & 72.9 \\
+ Gather-Excite \cite{gatherexcite}   &  77.6   & 81.3   & 72.6 \\
\rowcolor{LightCyan}
+ \ours    &  \bf{78.0}   & \bf{81.7}   & \bf{74.3} \\
\bottomrule
\end{tabular}
\end{table}

In \autoref{tab:Self100percImageNet}, we pre-train ResNet-50 and ViT-S using DINO \cite{dino} on the 100\% of ImageNet-1k for 100 epochs. SimPool brings an improvement of 1.8\% $k$-NN and \bill{.....} \emph{linear probing} with ResNet-50 and an improvement of 1.1\% $k$-NN and 1.3\% linear probing over baseline ViT-S. In \autoref{fig:SelfProbe}, ViT-S + SimPool achieves the same performance as ViT default with 90\% fewer training epochs.


\begin{figure}
\pgfplotsset{width=7cm,compat=1.9}
\begin{tikzpicture}
\small
\centering

\begin{axis}[
    xlabel=Epochs,
    ylabel=Validation Accuracy,
    legend style={at={(0.5,-0.15)},anchor=north},
    ymin=63,
    ymax=73,
    legend pos=outer north east
]
\addplot[smooth,blue] plot coordinates {
(0,63.6)
(10,70.4)
(20,70.9)
(30,71.1)
(40,71.3)
(50,71.4)
(60,71.4)
(70,71.5)
(80,71.5)
(90,71.5)
(100,71.5)
};
\addlegendentry{Default}

\addplot[smooth,red] plot coordinates {
(0,64.7)
(10,71.6)
(20,72.2)
(30,72.4)
(40,72.6)
(50,72.7)
(60,72.7)
(70,72.7)
(80,72.8)
(90,72.8)
(100,72.8)
};
\addlegendentry{SimPool}
\end{axis}
\end{tikzpicture}
\caption{\emph{Image classification} (top-1 accuracy, \%) on the 100\% of ImageNet-1k. Linear probing of ViT-S default vs. ViT-S + SimPool for 100 epochs.}
\label{fig:SelfProbe}
\end{figure}

\begin{table}[ht]
\small
\centering
\setlength{\tabcolsep}{3pt}
\caption{\emph{Image classification} (top-1 accuracy, \%) on the 100\% of ImageNet-1k. Self-supervised pretraining of ResNet-50 and and ViT-S for 100 epochs.}
\label{tab:Self100percImageNet}
\begin{tabular}{lcccc} 
\toprule
\mr{3}{\Th{Method}} & \mc{4}{\Th{Architecture}} \\  \cmidrule{2-5} 
 &  \mc{2}{\Th{ResNet-50}} & \mc{2}{\Th{ViT-S}} \\ \cmidrule{2-5}
 & \Th{$k$-NN} &\Th{Linear Prob} & \Th{$k$-NN} &\Th{Linear Prob} \\
\midrule
Default  &  62.2  &   \emph{running}   & 68.9 & 71.5 \\
\rowcolor{LightCyan}
+ \ours    &  \bf{64.0}  & \emph{running} & \bf{70.0} & ~\bf{72.8} \\
 %& \gp{+1.8\%}&& \gp{+1.1\%} & ~\gp{+1.3\%} \\
\bottomrule
\end{tabular}
\end{table}


%------------------------------------------------------------------------------
\begin{table}[ht]
\small
\centering
\setlength{\tabcolsep}{3pt}
\caption{\emph{Image classification} (top-1 accuracy, \%) on the 100\% of ImageNet-1k. Supervised training of ConvNeXt-s and ViT-S for 300 epochs.}
\label{tab:300percImageNet}
\begin{tabular}{lcc} \toprule
\mr{2}{\Th{Method}} & \mc{2}{\Th{Supervised}} \\  \cmidrule{2-3} 
 &  \Th{ConvNeXt-S}   & \Th{ViT-S} \\
\midrule
Default    &  83.1   &  77.9 \\
\rowcolor{LightCyan}
+ \ours    &  \bf{83.5}  &  \bf{78.7} \\
% & \gp{+0.4\%} & \gp{+0.8\%} &  \\
\bottomrule
\end{tabular}
\end{table}
%------------------------------------------------------------------------------

In \autoref{tab:300percImageNet}, we train ConvNeXt-S and ViT-S on the 100\% of ImageNet-1k for 100 epochs. ConvNeXt-S and ViT-S with SimPool bring an improvement of +0.4\%, +0.8\% over the baseline, respectively.

% resnet-18 -> 11.2
% resnet-50 -> 25.6
% vit-t -> 6.6
% vit-s -> 22.1
% convnext-s -> 50.0
% convnext-t -> 29.0




%------------------------------------------------------------------------------
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{3pt}
\caption{MaxBoxAccV2 on CUB test and ImageNet-1k val sets using ViT-S}
\label{tab:maxboxacc}
\begin{tabular}{lcccc} \toprule
\Th{Method} & \mc{2}{DINO pretrained} & \mc{2}{Supervised pretrained} \\ \midrule
& \Th{CUB} & \Th{ImageNet} & \Th{CUB} & \Th{ImageNet} \\ \midrule
Default & 82.71 & 61.99 & 63.12 & 53.60  \\
+ \ours & \bf{86.09} & \bf{66.07} & \bf{77.87} & \bf{64.38}  \\ \midrule 
 & \gp{+3.4\%} & \gp{+4.1\%} & ~\gp{+14.8\%} & ~\gp{+10.8\%}\\
\midrule 
Default @20 & 65.47 & 52.49 & 62.44 & 50.45  \\
+ \ours @20 & \bf{72.53} & \bf{58.73} & \bf{74.04} & \bf{62.59}  \\ \midrule
 & \gp{+7.0\%} & \gp{+6.2\%} & \gp{+21.6\%} & \gp{+12.1\%}  \\
\bottomrule
\end{tabular}
\end{table}
%-----------

%------------------------------------------------------------------------------
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{1pt}
\caption{CorLoc for object discovery using ViT-S as a backbone pretrained on ImageNet-1k with \gkako{DINO} for 100 epochs.}
\label{tab:corloc_lost}
\begin{tabular}{lccc|ccc} \toprule
\Th{Method} & \mc{3}{\Th{DINO-seg}~\cite{lost, dino}} & \mc{3}{\Th{LOST}~\cite{lost}} \\ \midrule
& \Th{VOC07} & \Th{VOC12} & \Th{COCO} & \Th{VOC07} & \Th{VOC12} & \Th{COCO} \\ \midrule
Default & 30.83 & 31.00 & 36.70 & 55.52 & 59.42 & 46.63  \\
+ \ours & \bf{53.22} & \bf{56.20} & \bf{43.41} & \bf{59.77} & \bf{65.02} & \bf{49.35} \\ \midrule
 & \gp{+22.4\%} & \gp{+25.2\%} & ~\gp{+16.7\%} & ~\gp{+4.3\%} & ~\gp{+5.6\%} & ~\gp{+2.8\%}\\
\midrule
Default @20 & 14.91 & 14.82 & 19.94 & 50.65 & 56.58 & 40.86 \\
+ \ours @20 & \bf{49.19} & \bf{54.79} & \bf{37.94} & \bf{53.90} & \bf{58.81} & \bf{46.08} \\ \midrule
 & \gp{+34.3\%} & \gp{+30.0\%} & ~\gp{+18.0\%} & ~\gp{+3.2\%} & ~\gp{+2.2\%} & ~\gp{+5.2\%}\\
\bottomrule
\end{tabular}
\end{table}
%-----------



\paragraph{Object localization}
Accurate localization is a critical aspect of deep learning models.
\billc{Indeed, localization can have a significant impact on the classification accuracy, particularly in situations where the input exhibit spatial variability or heterogeneity. Localization can help improve robustness.} \KK{[should the previous or the following]} When objects are partially occluded or have a complex background, localization is crucial for achieving high classification accuracy. If the localization is imprecise, the object's features may be distorted or mixed with other objects, leading to misclassification. Accurate localization is essential for ensuring the reliability of various applications. In \autoref{tab:maxboxacc}, we compare the localization performance of ViT-S with and without SimPool when pretrained supervised or self-supervised. We observe that SimPool brings significant improvement, and especially in the supervised case, it increases the localization by more than 10\% on MaxBoxAccV2. We highlight that even at epoch 20, it surpasses by 9\% the fully trained ViT-S. Moreover, SimPool increases the localization by over 3\% in the self-supervised setting.

In the same direction, we explore further the potential of SimPool to localize objects in images without supervision. Thus, we utilize the LOST~\cite{lost} method, which exploits the activation features of a vision transformer pre-trained using DINO for the unsupervised single-object discovery. Additionally, we experiment with the alternative baseline method DINO-seg~\cite{lost, dino} that leverages the attention maps to perform object localization. In \autoref{tab:corloc_lost}, SimPool significantly outperforms the default pretrained ViT-S for both object discovery methods on all three datasets. For DINO-seg, the improvement is more than 16.7\% and for LOST 2.8\%. Again, we observe that even at the first few epochs SimPools enables ViT-S to \KK{[deliver]} perform surprisingly good localization.



%------------------------------------------------------------------------------
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{1.8pt}
\caption{\emph{Background robustness}: On IN-9~\cite{xiao2021noise} and its variations. ViT-S supervised pretrained on ImageNet-1k}
\label{tab:BGChalsimpool}
\begin{tabular}{lcccccccc} \toprule
\Th{Method} &  OF & MS & MR & MN & NF & OBB & OBT & IN-9 \\ \midrule
\mc{9}{\Th{Supervised}} \\ \midrule
Default &  66.40 & 79.06 & 67.43 & 65.51 & 37.21 & 12.86 & 15.16 & 92.00 \\
+ \ours &  \bf{71.80} & \bf{80.20} & \bf{69.28} & \bf{67.33} & \bf{42.77} & \bf{15.19} & \bf{15.63} & \bf{92.94} \\\midrule
\mc{9}{\Th{DINO + Linear probing}} \\ \midrule
Default & \bf{87.26} & 87.88 & 78.49 & 76.72 & 47.85 & \bf{20.00} & \bf{16.94} & 95.3 \\
+ \ours &  \bf{87.26} & \bf{88.05} & \bf{80.59} & \bf{78.74} & \bf{48.17} & 17.78 & 16.72 & \bf{95.56} \\\bottomrule
\end{tabular}
\end{table}
%------------------------------------------------------------------------------


\paragraph{Background changes}

Deep neural networks often rely heavily on the background of an image, which can limit their ability to generalize well. To achieve better performance, these models must be able to cope with changes in the background and prioritize the foreground. To evaluate SimPool robustness to the background changes, we use the ImageNet-9~\cite{xiao2021noise} (IN-9) dataset. IN-9 contains nine coarse-grained classes with seven variations of both background and foreground. In four of these datasets, i.e., Only-FG (OF), Mixed-Same (MS), Mixed-Rand (MR), and Mixed-Next (MN), the background is modified. The three other datasets feature masked foregrounds, i.e., No-FG (NF), Only-BG-B (OBB), and Only-BG-T (OBT). In \autoref{tab:BGChalsimpool}, we show that SimPool guides ViT-S to be robust against background changes improving the scores for both supervised and self-supervised pretraining. We mention that SimPool with DINO pretraining does not increase scores only on OBB and OBT, which is preferable given that none of the foreground objects or masks are present in these settings.



%------------------------------------------------------------------------------
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{1pt}
\caption{\emph{Image retrieval} (mAP, \%) on (a) $\cR$Oxford and (b) $\cR$Paris~\cite{radenovic2018revisiting}. ViT-S models pre-trained with DINO on ImageNet-1k training set for 100 epochs.}
\label{tab:100percDownStreamRox}
\begin{tabular}{lcc|cc} \toprule
\mr{2}{\Th{Backbone}} & \mc{2}{(a) \Th{$\cR$Oxford}} & \mc{2}{(b) \Th{$\cR$Paris}}                     \\ \cmidrule{2-5}
                    & \Th{Medium} & \Th{Hard}  & \Th{Medium} & \Th{Hard}    \\ \midrule
%             \mc{5}{Supervised}       \\ \midrule
%ViT-S              & 23.05    & \bf{6.55}      & \bf{55.07}        & \bf{27.09}          \\
%ViT-S+SimPool          & \bf{23.68}   & 5.58  & 54.23   & 26.89  \\ \midrule
%             \mc{5}{DINO}       \\ \midrule
ResNet-50              & 27.18    & 7.88       & 47.28        & 18.95           \\
ResNet-50 + SimPool          & \bf{29.71}   & \bf{8.69}  & \bf{51.56}   & \bf{22.99}  \\\midrule
ViT-S              & 29.43    & 10.02       & 54.56        & 26.22           \\
ViT-S + SimPool          & \bf{32.08}   & \bf{10.58}  & \bf{56.48}   & \bf{27.28}  \\
\bottomrule
\end{tabular}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{2.5pt}
\caption{\emph{Image classification} (accuracy, \%) on CIFAR-10 \cite{cifar}, CIFAR-100 \cite{cifar} and Oxford Flowers \cite{oxford_flowers}. ViT-S models pre-trained with DINO on ImageNet-1k training set for 100 epochs.}
\label{tab:finetuning}
\begin{tabular}{lccc} \toprule
 & (a) \Th{CIFAR-10} & (b) \Th{CIFAR-100} & (c) \Th{Flowers} \\ \midrule
Default & 98.7 & 89.8 & 97.8  \\
\ours & \bf{98.9} & \bf{89.9} & \bf{98.4}  \\ \midrule 
 & \gp{+0.2\%} & \gp{+0.1\%} & ~\gp{+0.6\%} \\
\bottomrule
\end{tabular}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{2.5pt}
%\caption{\Comparing ViT-S.}
\label{tab:efficiency}
\begin{tabular}{lcccc} \toprule
 & \Th{Depth} &\Th{Init Layer} & \Th{Accuracy} & \Th{\#params} \\ \midrule
ViT-S $\cls$ & 12 & 0 & 72.7  & 22.1M \\
ViT-S GAP & 12 & 12 & 73.3  & 22.1M \\ \midrule
ViT-S $\cls$ & 13 & 0 & 73.2  & 23.8M \\ 
ViT-S $\cls$ & 14 & 0 & 73.7  & 23.8M \\
ViT-S $\cls$ & 15 & 0 & -  & 23.8M \\\midrule
ViT-S + SimPool & 12 & 12 & \bf{74.3}  & 22.3M\\
ViT-S + SimPool & 11 & 12 & \bf{74.0}  & 20.6M\\
ViT-S + SimPool & 10 & 12 & \bf{73.6}  & 18.7M\\
ViT-S + SimPool & 9 & 12 & 72.5  & 17.0M\\
\bottomrule
\end{tabular}
\end{table}
%------------------------------------------------------------------------------


\paragraph{Downstream on image retrieval}

While classification accuracy indicates the model's ability to recognize objects in an image, it does not necessarily reflect its ability to capture the visual similarity between images. Here, we examine the understanding of the visual features across different images learned with SimPool along with ResNet-50 and ViT-S on image retrieval. In \autoref{tab:100percDownStreamRox}, we observe that SimPool is very effective on $\cR$Oxford and $\cR$Paris~\cite{radenovic2018revisiting} enhancing the scores for all models and protocols combinations.



==> tex/exp-bench-sub.tex <==
\subsection{Benchmark}
\label{sec:bench}

\paragraph{Image Classification}

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
\toprule
\Th{Method} & \Th{ResNet-50} & \Th{ConvNeXt-S} & \Th{ViT-S} \\
\midrule
Baseline   &  77.4   & 81.1   & 72.7 \\
CaiT \cite{cait}    &  77.3   & 81.2   & 72.6 \\
Slot \cite{slot}    & 77.3   & 80.9 & 72.9 \\
Gather-Excite \cite{gatherexcite}   &  77.6   & 81.3   & 72.6 \\
\rowcolor{LightCyan}
\Ours    &  \bf{78.0}   & \bf{81.7}   & \bf{74.3} \\
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{\emph{Image classification} top-1 accuracy \% on ImageNet-1k. Supervised pre-training for 100 epochs. Best competitors selected per group from \autoref{fig:tourn}.}
\label{tab:Super100percImageNet}
\end{table}
%------------------------------------------------------------------------------

\autoref{tab:Super100percImageNet} compares \Ours with the tournament winners per group of \autoref{sec:analysis} on supervised pre-training for classification. \Ours outperforms all methods, consistently improving the baseline by 0.6\% using convolutional networks and by 1.6\% using ViT. Gather-Excite~\cite{gatherexcite} improves over the baseline only on convolutional networks, while Slot~\cite{slot} only on ViT-S. CaiT improves over the baseline only for ConvNeXt-S. By contrast, \Ours improves everywhere.

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcccccc}
\toprule
\mr{2}{\Th{Method}} &  \mc{2}{\Th{ResNet-50}} & \mc{2}{\Th{ConvNeXt-S}} & \mc{2}{\Th{ViT-S}} \\ \cmidrule{2-7}
& \Th{$k$-NN} &\Th{Prob} & \Th{$k$-NN} &\Th{Prob} & \Th{$k$-NN} &\Th{Prob} \\
\midrule
Baseline  &  62.2 & 64.4 & 59.3 & & 68.9 & 71.5 \\
\rowcolor{LightCyan}
\Ours    &  \bf{63.9}  & \bf{66.7} & & & \bf{69.9} & ~\bf{72.8} \\
 %& \gp{+1.8\%}&& \gp{+1.1\%} & ~\gp{+1.3\%} \\
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{\emph{Image classification} top-1 accuracy, \% on ImageNet-1k. Self-supervised pre-training with DINO~\cite{dino} for 100 epochs.}
\label{tab:Self100percImageNet}
\end{table}
%------------------------------------------------------------------------------

\autoref{tab:Self100percImageNet} evaluates self-supervised pre-training. \Ours improves over the baseline by (a) 1.7\% $k$-NN and 2.3\% linear probing on ResNet-50; (b) 1.0\% $k$-NN and 1.3\% linear probing on ViT-S.

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc} \toprule
\Th{Method} &  \Th{ResNet-50} & \Th{ConvNeXt-S}   & \Th{ViT-S} \\
\midrule
Baseline & 78.1 &  83.1   &  77.9 \\
\rowcolor{LightCyan}
\Ours & \bf{78.7} &  \bf{83.5}  &  \bf{78.7} \\
% & \gp{+0.4\%} & \gp{+0.8\%} &  \\
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{\emph{Image classification} top-1 accuracy \% on ImageNet-1k. Supervised pre-training of ConvNeXt-S, ViT-S for 300 epochs; ResNet-50 for 200 epochs.}
\label{tab:300percImageNet}
\end{table}
%------------------------------------------------------------------------------

\autoref{tab:300percImageNet} evaluates supervised pre-training for classification for 300 epochs. \Ours improves over the baseline by 0.4\% accuracy on ConvNeXt-S and 0.8\% on ViT-S.

% resnet-18 -> 11.2
% resnet-50 -> 25.6
% vit-t -> 6.6
% vit-s -> 22.1
% convnext-s -> 50.0
% convnext-t -> 29.0

%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lccc} \toprule
\Th{Method} & \Th{CIFAR-10}~\cite{cifar} & \Th{CIFAR-100}~\cite{cifar} & \Th{Flowers}\cite{oxford_flowers} \\ \midrule
Baseline & 98.7 & 89.8 & 98.3  \\
\rowcolor{LightCyan}
\Ours & \bf{98.9} & \bf{89.9} & \bf{98.4}  \\
%\gain{
%\midrule
% & \gp{+0.2\%} & \gp{+0.1\%} & ~\gp{+0.6\%} \\
 %}
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{\emph{Image classification} accuracy \%, finetuning for classification for 1000 epochs. ViT-S self-supervised pre-training with DINO~\cite{dino} on ImageNet-1k for 100 epochs.}
\label{tab:finetuning}
\end{table}
%------------------------------------------------------------------------------

\paragraph{Fine-tuning for classification}

\autoref{tab:finetuning} evaluates finetuning for classification on different datasets of a self-supervised ViT. \Ours brings small improvement over the baseline in all cases.

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcccc} \toprule
\mr{2}{\Th{Method}} & \mc{2}{\Th{Self-supervised}} & \mc{2}{\Th{Supervised}} \\ \cmidrule{2-5}
& \Th{CUB} & \Th{ImageNet} & \Th{CUB} & \Th{ImageNet} \\ \midrule
Baseline & 82.71 & 61.99 & 63.12 & 53.60  \\
\rowcolor{LightCyan}
\ours & \bf{86.09} & \bf{66.07} & \bf{77.87} & \bf{64.38}  \\
\gain{
\midrule
 & \gp{+3.4\%} & \gp{+4.1\%} & ~\gp{+14.8\%} & ~\gp{+10.8\%}\\
}
\midrule
Baseline@20 & 65.47 & 52.49 & 62.44 & 50.45  \\
\rowcolor{LightCyan}
\ours@20 & \bf{72.53} & \bf{58.73} & \bf{74.04} & \bf{62.59}  \\
\gain{
\midrule
 & \gp{+7.0\%} & \gp{+6.2\%} & \gp{+21.6\%} & \gp{+12.1\%}  \\
}
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{\emph{Localization accuracy} MaxBoxAccV2 on CUB test set and ImageNet-1k validation set. ViT-S pre-trained on ImageNet-1k for 100 epochs. Self-supervision with DINO~\cite{dino}.}
\label{tab:maxboxacc}
\end{table}
%------------------------------------------------------------------------------

\paragraph{Object localization}

Accurate localization can have a significant impact on the classification accuracy, particularly under multiple objects, complex scenes and background clutter. \autoref{tab:maxboxacc} evaluates localization accuracy under both supervision settings. \Ours significantly improves the baseline, by up to 7\% MaxBoxAccV2 when self-supervised and up to 14\% when supervised. In the latter case, the gain is already up to 12\% at epoch 20.

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{lccc|ccc} \toprule
\mr{2}{\Th{Method}} & \mc{3}{\Th{DINO-seg}~\cite{lost, dino}} & \mc{3}{\Th{LOST}~\cite{lost}} \\ \cmidrule{2-7}
& \Th{VOC07} & \Th{VOC12} & \Th{COCO} & \Th{VOC07} & \Th{VOC12} & \Th{COCO} \\ \midrule
Baseline & 30.83 & 31.00 & 36.70 & 55.52 & 59.42 & 46.63  \\
\rowcolor{LightCyan}
\ours & \bf{53.22} & \bf{56.20} & \bf{43.41} & \bf{59.77} & \bf{65.02} & \bf{49.35} \\
\gain{
\midrule
 & \gp{+22.4\%} & \gp{+25.2\%} & ~\gp{+16.7\%} & ~\gp{+4.3\%} & ~\gp{+5.6\%} & ~\gp{+2.8\%}\\
}
\midrule
Baseline@20 & 14.91 & 14.82 & 19.94 & 50.65 & 56.58 & 40.86 \\
\rowcolor{LightCyan}
\ours@20 & \bf{49.19} & \bf{54.79} & \bf{37.94} & \bf{53.90} & \bf{58.81} & \bf{46.08} \\
\gain{
\midrule
 & \gp{+34.3\%} & \gp{+30.0\%} & ~\gp{+18.0\%} & ~\gp{+3.2\%} & ~\gp{+2.2\%} & ~\gp{+5.2\%}\\
}
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{\emph{Object discovery} CorLoc. ViT-S pre-trained with DINO~\cite{dino} self-supervision on ImageNet-1k for 100 epochs.}
\label{tab:corloc_lost}
\end{table}
%------------------------------------------------------------------------------

\paragraph{Unsupervised object discovery}

\autoref{tab:corloc_lost} studies LOST \cite{lost}, which uses the raw features of a vision transformer pre-trained using DINO~\cite{dino} for unsupervised single-object discovery, as well as the baseline DINO-seg~\cite{lost, dino}, which uses the attention maps instead. \Ours significantly outperforms the baseline on all datasets, by up to 25.2\% CorLoc for DINO-seg and 5.6\% for LOST, on VOC12. Again, the gain is significant already at the first 20 epochs.

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lcccccccc} \toprule
\Th{Method} &  OF & MS & MR & MN & NF & OBB & OBT & IN-9 \\ \midrule
\mc{9}{\Th{Supervised}} \\ \midrule
Baseline &  66.40 & 79.06 & 67.43 & 65.51 & 37.21 & 12.86 & 15.16 & 92.00 \\
\rowcolor{LightCyan}
\Ours &  \bf{71.80} & \bf{80.20} & \bf{69.28} & \bf{67.33} & \bf{42.77} & \bf{15.19} & \bf{15.63} & \bf{92.94} \\\midrule
\mc{9}{\Th{DINO~\cite{dino} Self-supervised + Linear probing}} \\ \midrule
Baseline & \bf{87.26} & 87.88 & 78.49 & 76.72 & 47.85 & \bf{20.00} & \bf{16.94} & 95.3 \\
\rowcolor{LightCyan}
\Ours &  \bf{87.26} & \bf{88.05} & \bf{80.59} & \bf{78.74} & \bf{48.17} & 17.78 & 16.72 & \bf{95.56} \\\bottomrule
\end{tabular}
\vspace{3pt}
\caption{\emph{Background robustness} on IN-9~\cite{xiao2021noise} and its variations; more details in the appendix. ViT-S pre-training on ImageNet-1k for 100 epochs.}
\label{tab:BGChalsimpool}
\end{table}
%------------------------------------------------------------------------------

\paragraph{Background changes}

We evaluate robustness to the background changes using IN-9~\cite{xiao2021noise} dataset, which contains nine coarse-grained classes with seven variations of background and foreground; more details are in the appendix. \autoref{tab:BGChalsimpool} shows that \Ours improves over the baseline under both supervision settings with only 2 out of 8 exceptions under DINO~\cite{dino} pretraining. The latter is justified given that none of the foreground objects or masks are present in these settings.

%------------------------------------------------------------------------------
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccccc} \toprule
\Th{Network}          & \Th{Pooling}  & \Th{Depth} &\Th{Init} & \Th{Accuracy} & \Th{\#params} \\ \midrule
\textsc{Base}         & GAP           & 12 & 12 & 73.3  & 22.1M \\ \midrule
\textsc{Base}         & \mr{5}{\cls}  & 12 & 0 & 72.7  & 22.1M \\
$\textsc{Base} + 1$   &               & 13 & 0 & 73.2  & 23.8M \\
$\textsc{Base} + 2$   &               & 14 & 0 & 73.7  & 25.6M \\
$\textsc{Base} + 3$   &               & 15 & 0 & 73.8  & 27.4M \\
$\textsc{Base} + 4$   &               & 16 & 0 & \bf{-}  & -M \\\midrule
\textsc{Base}         & \mr{4}{\ours} & 12 & 12 & \bf{74.3}  & 22.3M\\
$\textsc{Base} - 1$   &               & 11 & 11 & 74.0  & 20.6M\\
$\textsc{Base} - 2$   &               & 10 & 10 & 73.6  & 18.7M\\
$\textsc{Base} - 3$   &               & 9 & 9 & 72.5  & 17.0M\\
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{\emph{Trade-off between performance and parameters}; supervised pre-training of ViT-S on \imagenet for 100 epochs. \Th{Init}: Initial layer of pooling token. \textsc{Base}: original network. \textsc{Base}$+b$ (\textsc{Base}$-b$): $b$ blocks added to (removed from) the network.}
\label{tab:param}
\end{table}
%------------------------------------------------------------------------------

\paragraph{Performance \vs parameters}

\autoref{tab:param} aims to answer the question of how much the performance improvement of \Ours is due to parameters of the query and key mappings. Interestingly, ViT-S works better with GAP than the default \cls. \Ours adds 0.2M parameters to the network. For fair comparison, we remove blocks from the network (\Th{Base}) when using \Ours and add blocks when using $\cls$. We find that, to achieve the same accuracy as \Th{Base} \Ours, \Th{Base} $\cls$ needs 3 extra blocks, \ie, 5M more parameters. Equally interestingly, removing 3 blocks from \Th{Base} \Ours is only slightly worse than \Th{Base} \cls, having 5M fewer parameters.

==> tex/exp-setup-1.tex <==
\section{Experiments}
\label{sec:exp}

\subsection{Setup}
\label{sec:setup}

%------------------------------------------------------------------------------

\paragraph{Datasets, Networks and Evaluation Protocol}

We perform supervised \emph{image classification} on ImageNet-1k using ResNet-18, ResNet-50 \cite{resnet}, ConvNeXt-S \cite{convnext}, ViT-T and ViT-S \cite{vit}. For the experimental analysis \autoref{sec:analysis} and ablation \autoref{sec:ablation}, we train ResNet-18 on the 20\% of ImageNet-1k \cite{imagenet} for 100 epochs. We train using the first 20\% of training samples per class and evaluate on the original validation set. For benchmark \autoref{sec:bench} we train ResNet-50, ConvNeXt-S-S and ViT-S on the 100\% of ImageNet-1k for 100 epochs; ResNet-50 and ConvNeXt-S on the 100\% of ImageNet-1k for 300 epochs. We measure top-1 classification accuracy.

We perform self-supervised \emph{pretraining} on the 100\% of ImageNet-1k using DINO \cite{dino} with ResNet-50 and ViT-S for 100 epochs, DINO with ViT-S for 300 epochs. We evaluate on ImageNet-1k validation set by $k$-NN or \emph{linear probing}. For \emph{linear probing}, we train a linear classifier on top of features as in DINO \cite{dino}. For $k$-NN \cite{instancediscrimination}, we freeze the pretrained model and extract features of training images, then use a $k$-nearest neighbor classifier with $k = 20$.

We downstream both supervised and self-supervised models to others tasks, either with or without \emph{finetuning}. We validate \emph{robustness} against background changes using ViT-S on ImageNet-9 \cite{xiao2021noise} and its variations. We use the linear head and the linear probe for supervised and self-supervised ViT-S respectively. We measure classification accuracy. We perform \emph{object localization} without finetuning using both supervised and self-supervised ViT-S on CUB \cite{CUB} and ImageNet-1k. We report MaxBoxAccV2 \cite{wsol}. We validate self-supervised ViT-S without finetuning on VOCC07 \cite{voc}, VOC12 \cite{voc} and COCO \cite{coco} for \emph{object discovery} using DINO-SEG \cite{dino} and LOST \cite{lost}. We report CorLoc \cite{corloc}. We finetune self-supervised ViT-S on CIFAR-10 \cite{cifar}, CIFAR-100 \cite{cifar} and Oxford Flowers \cite{oxford_flowers} for \emph{image classification} measuring top-1 classification accuracy. Without finetuning, we extract features as with $k$-NN for both self-supervised ResNet-50 and ViT-S and validate on revisited $\cR$Oxford and $\cR$Paris~\cite{radenovic2018revisiting} for \emph{image retrieval} measuring mAP~\cite{radenovic2018revisiting}.

In Supplementary, we provide more benchmarks, visualizations and ablations.

\paragraph{Implementation details}

Exhaustive implementation details are given in the Supplementary.

%For HOW we use a kernel of size 3 and we do not perform dimensionality reduction. For LSE we initialize $r=10$ . For GeM we use a kernel of size 7 and initialize $gamma=2$.

==> tex/intro-1.tex <==
\section{Introduction}
\label{sec:intro}

1. Are we gonna sell it as a pooling or feature re-weighting mechanism? Are we gonna explain that these two at the end of the day are the same thing? No matter what, I see two different ways of starting the story:

a. Why pooling matters? This is the question we ask here. We could start saying some things about poolings and some good properties that a pooling should have given a specific task. 

b. We start the story from Vision Transformers. We slightly highlight the differences between Vision Transformers and CNNs (receptive field, etc.). We can argue that the two main components of Vision Transformers are: (i) the multi-head self-attention mechanism and the (ii) [CLS] token. 

We say some thing about multi-head self-attention. Maybe compare it with cross-attention. 

Also, some things about the [CLS], like: The [CLS] token encodes information from the previous layers and the self attention mechanism chooses (for the final layer) which information to aggregate (other patch tokens from the last layer and [CLS] token). We argue that because of the fact that Vision Transformers were inspired by NLP, the concept of [CLS] token was directly brought to CV. Thus, while in the era of CNNs, a great study around pooling mechanisms had be done in retrieval, classification, etc, the same \emph{does not hold} for Vision Transformers (under-studied). Few works have tried to do something different (than [CLS]): GAP \cite{swin, rest, halonet} or attention pooling \cite{clip}. In this paper, we doubt about the need of having a [CLS] token interacting with all the other tokens from the start of the network.

We propose a new mechanism/strategy that utilizes attention to create an universal cross-network global representation. In order to do so, we reformulate the existing pooling mechanisms/strategies under a generic framework. This helps recognizing their differences (and similarities) and gaining useful insight. 

Other pooling strategies:
CBAM \cite{cbam}, LogSumExp \cite{lse}, BlurPool \cite{blurpool}, i-sqrt cov\cite{isqrtcov}, Gather-Excite \cite{gatherexcite}, DELF \cite{delf}, DELG \cite{delg}, HOW \cite{how}, OTK \cite{otk}, SOLAR \cite{solar}, UOT \cite{uot}, PSWE \cite{pswe}, OTK \cite{otk}, GSOP \cite{gsop}, Kernel Pooling\cite{kernelpooling}, WELDON \cite{weldon}

 Our strategy improves the performance of the network by allowing it to selectively attend to different regions of the feature map (i.e. there is no transformation in features). 

\begin{itemize}
    \item We reformulate the existing pooling mechanisms and encompass them under a generic framework.
    \item We perform extensive experiments on bla bla.
    \item We find that under different scenarios and models, our strategy is able to boost the performance up to $2\%$.
    \item We present valuable insights/analysis/properties.
\end{itemize}

We have to discuss about those properties and compare with other competitors to see exactly where we are. I was thinking properties like:

1. quantitatively to show that our first-epoch attention maps are good (we've seen this qualitatively)
2. maybe extract features from one of our network and runs k-means on top. compare this with the mult-ihead self-attention. which one is better?
3. show some things about gamma and how this affects attention
4. qualitatively to show how good are our attention maps in general
5. show localization properties 

------------------------------------------------------

"Due to the success of transformers in NLP tasks, vision transformers were proposed as a way to apply the transformer architecture to computer vision tasks. Inspired by the use of the [CLS] token in NLP, which provides a fixed-length representation of the entire input sequence, vision transformers also introduced a similar concept of a [CLS]-like token for images. This token serves as a summary representation of the entire image and is used for downstream tasks, such as image classification or object detection."

During the forward pass of the transformer, the CLS token is added to the input sequence as a special token. The output representation of the CLS token after passing through the transformer is used as the fixed-length representation of the entire sequence. 

Our main contributions probably are the use of cross-attention in image classification + an attention-weighted generalized mean + emerging properties and analysis.
%is fully devoted to summarizing the information to be fed to the linear classifier.


==> tex/method-1.tex <==
\section{Method v1}
\label{sec:1:method}

\begin{figure*}[t]
\centering
\fig[0.95]{method/overview.pdf}
\caption{Overview of [GAP-CLS]
}
\label{fig:1:overview}
\end{figure*}
%------------------------------------------------------------------------------


\subsection{GAP-CLS}
%Let $I \in \mathbb{R}^{W\times H\times 3}$ be the input image to a backbone network, where $W, H$ are the spatial dimensions

Let $X \in \mathbb{R}^{W \times H \times D}$ be the $3$-dimensional \emph{feature} tensor from the last layer of a network, where $W, H$ are the spatial dimensions and $D$ the number of channels. Let $X_{i,j,k}$ denote the entry in $X$ that corresponds to channel $k$, at spatial location $(i,j)$. We initialize the classification token [CLS] \cite{transformer} by applying \emph{global average pooling} on the feature tensor as:
\begin{align}
    [CLS]_{init} = \frac{1}{WH}\sum_{i=1}^{W}\sum_{j=1}^{H}X_{i,j}
\label{eq:1:cls_init}
\end{align}
The [CLS] token is used a 

\begin{align}
        Q  = W_q [CLS]_{init}
\label{eq:1:q_linear}
\end{align}

\begin{align}
	K = W_k X
 \label{eq:1:k_linear}
\end{align}

\begin{align}
	A = \softmax \left( Q K\tran / \sqrt{D} \right).
\label{eq:1:att}
\end{align}

$\forall X_{i,j,k} \in \mathbb{R^{+}}$:

\begin{align}
    [CLS]_{refined} = (A X^{\circ{\gamma}} )^{\circ{1/\gamma}}
\label{eq:1:att_lp_pool}
\end{align}

If $\exists X_{i,j,k} \in \mathbb{R^{-}}$:

\begin{align}
    [CLS]_{refined} = (A (X - min(X_{i,j,k})) ^{\circ{\gamma}} )^{\circ{1/\gamma}} + \beta 
\label{eq:1:att_lp_pool-min}
\end{align}

==> tex/plots-ext.tex <==
%------------------------------------------------------------------------------
% hack for CVPR/ICCV style
\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother

%------------------------------------------------------------------------------
% main packages
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{tikzextern}
\usepackage{pgffor}

%------------------------------------------------------------------------------
% externalization
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/plots-none.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/related-1.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Pooling}

The pooling operation is highly related to convolutional networks, studied mainly under instance-level tasks \cite{crow, delf, delg, how, solar} and less under category-level tasks \cite{se, cbam, gatherexcite, gsop, nln}. Starting before deep learning \cite{fast-spatial, sift, vlad, asmk}, pooling can be \emph{spatial} \cite{gatherexcite, crow, delf, delg, how, solar}, \emph{channel} \cite{se, gsop, crow} or both \cite{cbam, crow}, \emph{local} \cite{se, crow, delf, how} or \emph{global} \cite{nln, aa_net, a2_net, san, n3_net}. 

Pooling can produce single or multiple \cite{otk} vectors.

Pooling can be non-trainable \cite{nin, mac}.

GAP is proposed in \cite{theor}, gap+max in \cite{gapmax} and an early attention pooling in \cite{gatedatt}.

Other pooling strategies: spatial pyramid pooling \cite{spp},
 BlurPool \cite{blurpool}, i-sqrt cov\cite{isqrtcov}, PSWE \cite{pswe}, Kernel Pooling\cite{kernelpooling}, WELDON \cite{weldon}.

The story might go like: the poolings are related to CNNs. There are those different kind of poolings, bla bla. Maybe put the following categories: spatial, channel, local, global, parameter-free, learnable. Then we say specifically about learnable poolings and highlight some attention-based pooling examples. We also mention feature reweighting methods can also be part of it; with only difference the lack of sum at the end. Then we say that pooling in convolutional networks was both inside the network and at the end. We say about the property of global pooling as an operation of information fusion to make the representation invariant to input permutations.

\paragraph{Vision Transformers}

Contrary to convolutional networks, transformers downsample only at input. Inside the network, a form of attention-pooling or better-stated feature reweighting is been done using a self-attention mechanism. There are a lot of works that have focused on improving the token (attention) mixing mechanism of transformers. Examples: shifting windows \cite{swin}, refining attention maps \cite{refiner, spatialentropy, intriguing}, relative position encoding \cite{rethinking}, introducing convolutions \cite{convit}, MLP spatial mixing instead of attention mixing \cite{resmlp} or even simple pooling instead of attention \cite{metaformer}.

The ones that refine attention maps:
\begin{itemize}
    \item \cite{spatialentropy} integrates a spatial entropy loss in order to produce attention maps which focus on local regions.
    \item \cite{intriguing} introduces a new shape token and adapts attentive distillation to distill shape knowledge from a CNN.
    \item \cite{refiner} directly refines the attention maps by projecting them to a higher dimensional space to promote their divesity
\end{itemize}

Shashank's work \cite{skip} does not directly refines the attention maps. The main goal is efficiency. It's a regularization.

Few works have tried to do something different (than [CLS]): GAP \cite{swin, rest, halonet} or attention pooling \cite{clip}. 

\cite{cnnvsvit} here they examine the differences between CNNs and transformers. they say that when trained with GAP, ViTs show less clear localization, but they use JFT-300M for this.


==> tex/related-2.tex <==
\section{Related Work}
\label{sec:related}

Spatial pooling of visual input is the process by which spatial resolution is reduced to $1 \times 1$, such that the input is mapped to a single vector. This process can be gradual and interleaved with mapping to a feature space, because any feature space is amenable to smoothing by spatial interactions or downsampling. The objective is robustness to deformation while preserving important visual information.

\paragraph{Background}

The study of receptive fields in neuroscience~\cite{receptive} lead to the development of 2D \emph{Gabor filters}~\cite{gabor} as a model of the first processing layer in the visual cortex. Visual descriptors based on filter banks in the frequency domain~\cite{gist} and orientation histograms~\cite{sift, hog} can be seen as efficient implementations of the same idea. Apart from mapping to a new space---that of filter responses or orientation bins---they involve a form of smoothing, at least in some orientation, and weighted local spatial pooling.

\emph{Textons}~\cite{texton1} can be seen as a second layer, originally studied in the context of texture discrimination~\cite{texture} and segmentation~\cite{texton1, texton2} and taking the form of multidimensional histograms on Gabor filter responses. The \emph{bag of words} model~\cite{bow-r, bow-c} is based on the same idea, as a histogram on other visual descriptors. Again, apart from mapping to a new space---that of textons or visual words---they involve local or global spatial pooling.

\emph{Histograms} and every step of building visual features can be seen as a form of nonlinear coding followed by pooling~\cite{code-pool}. \emph{Coding} is maybe the most important factor. For example, a high-dimensional mapping before pooling, optionally followed by dimension reduction after pooling, can reduce interference between elements~\cite{fisher, vlad, emk}. \emph{Weighting} of individual elements is also important in attending important regions~\cite{spp, recept-learn, auto-pool} and in preventing certain elements from dominating others~\cite{burst, gmp, demo}.

The \emph{pooling operation} itself is any symmetric (permutation-invariant) set function of the form $f(X) = g\left(\sum_{x \in X} f(x)\right)$~\cite{deep-sets}, with the most common being average and maximum~\cite{hmax, theor, code-pool}. Apart from a single vector, one may obtain \emph{multiple vectors} based on a spatial partition~\cite{spp} or a partition in the feature space~\cite{he, asmk}, but this requires a particular kernel for matching.

%------------------------------------------------------------------------------

\paragraph{Convolutional networks}

Following findings of neuroscience, early convolutional networks~\cite{neo, lenet} are based on learnable \emph{convolutional layers} interleaved with fixed \emph{spatial pooling layers} that downsample, which is an instance of the coding-pooling framework. The same design remains until today~\cite{alexnet, vgg, resnet, convnext}. Again, apart from mapping to a new space, convolutional layers involve a form of weighted local pooling. Again, the operation in pooling layers is commonly average~\cite{lenet} or maximum~\cite{hmax, alexnet}.

Early networks end in a fully-connected layer over a feature tensor of low resolution~\cite{lenet, alexnet, vgg}. This evolves into spatial pooling, \eg global / regional average followed by a classifier for category-level tasks like classification~\cite{nin, resnet} / detection~\cite{frcnn}, or global maximum followed by a pairwise loss~\cite{mac} for instance-level tasks. This is beneficial for downstream tasks and interpretability~\cite{cam}.

The spatial pooling operation at the end of the network is widely studied in instance level-tasks~\cite{spoc, mac, gem}, giving rise to forms of \emph{spatial attention}~\cite{crow, delf, delg, how, solar}, In category-level tasks, it is more common to study \emph{feature re-weighting} as components of the architecture~\cite{se, cbam, gatherexcite}. The two are closely related because \eg the weighted average is element-wise weighting followed by sum. Most modern pooling operations are learnable.

Pooling can be \emph{spatial}~\cite{gatherexcite, delf, delg, how, solar}, \emph{over channels}~\cite{se}, or both \cite{crow, cbam}. CBAM~\cite{cbam} is particularly related to our work in the sense that it includes global average pooling followed by a form of spatial attention, although the latter is not evident in its original formulation and although CBAM is a feature re-weighting rather than pooling mechanism.

Apart from a single vector, one may obtain \emph{multiple vectors} \eg by some form of clustering~\cite{diffuse} or optimal transport~\cite{otk}. This however requires a particular kernel for matching and is outside the scope of this work.

%------------------------------------------------------------------------------

\paragraph{Vision transformers}

\emph{Pairwise interactions} between features are forms of pooling that can be seen as alternatives to convolution or forms of self-attention. Most have been designed as architectural components of convolutional networks, again over the spatial~\cite{nln, aa_net, san, n3_net} or the channel dimensions~\cite{a2_net, eca}. Originating in language models~\cite{transformer}, \emph{vision transformers}~\cite{vit} streamlined these approaches and became the dominant competitors of convolutional networks. Several variants often bring back ideas from convolutional networks, including spatial hierarchy~\cite{swin}, relative position encoding~\cite{rethinking, levit}, re-introducing convolution~\cite{cvt,convit}, re-introducing pooling layers~\cite{pit}, or simple pooling instead of attention~\cite{metaformer}.

Transformers downsample only at the input, forming spatial \emph{patch tokens}. Pooling is based on a learnable \cls (``classification'') token, which, beginning at the input space, undergoes the same self-attention operation with patch tokens and eventually provides a global image representation. That is, the network ends in global weighted average pooling, using as weights the attention of \cls over the patch tokens. Pooling is still gradual, since \cls interacts with patch tokens throughout the network depth.

Few works that have studied anything other than \cls for pooling in transformers are mostly limited to global average pooling (GAP)~\cite{swin, rest, halonet, cnnvsvit}. \cls offers attention maps for free, but those are typically of low quality unless in a self-supervised setting~\cite{dino}, which is not well understood. Few works that attempt to rectify this in the supervised setting include a spatial entropy loss~\cite{spatialentropy}, shape distillation from convolutional networks~\cite{intriguing} and skipping computation of self-attention~\cite{skip}.

We attempt to address these limitations and study pooling in convolutional networks, vision transformers, supervised and self-supervised settings alike. We derive a simple, attention-based, universal pooling mechanism that applies equally to all cases, improving both performance and attention maps. To our knowledge, we are the first to obtain attention maps in supervised transformers of at least as good quality as self-supervised, without modifying the architecture.


% \paragraph{Pooling}

% \cite{bilinear, compact-bilinear}
% GAP is proposed in \cite{theor}, gap+max in \cite{gapmax} and an early attention pooling in \cite{gatedatt} -> deep sets.
% BlurPool \cite{blurpool}, i-sqrt cov\cite{isqrtcov}, PSWE \cite{pswe}, Kernel Pooling\cite{kernelpooling}, WELDON \cite{weldon}.

% \paragraph{Vision Transformers}

% MLP spatial mixing instead of attention mixing \cite{resmlp} 
% attention pooling \cite{clip}. 
% \cite{cnnvsvit} here they examine the differences between CNNs and transformers. they say that when trained with GAP, ViTs show less clear localization, but they use JFT-300M for this.
% \cite{refiner} directly refines the attention maps by projecting them to a higher dimensional space to promote their divesity


==> tex/related-3.tex <==
\section{Related Work}
\label{sec:related}

% Spatial pooling of visual input is the process by which spatial resolution is reduced to $1 \times 1$, such that the input is mapped to a single vector. This process can be gradual and interleaved with mapping to a feature space, because any feature space is amenable to smoothing by spatial interactions or downsampling. The objective is robustness to deformation while preserving important visual information.

\paragraph{Background}

The study of receptive 
fields~\cite{receptive} 
% fields in neuroscience~\cite{receptive} 
lead to the development of 2D \emph{Gabor filters}~\cite{gabor} as a model of the first processing layer in the visual cortex. Visual descriptors based on filter banks in the frequency domain~\cite{gist} and \emph{orientation histograms}~\cite{sift, hog} can be seen as efficient implementations of the same idea. Apart from mapping to a new space---that of filter responses or orientation bins---they involve 
% a form of smoothing, at least in some orientation, and 
weighted local spatial pooling.

\emph{Textons}~\cite{texton1, texton2} can be seen as a second layer, 
% \emph{Textons}~\cite{texton1} can be seen as a second layer, 
% originally studied in the context of texture discrimination~\cite{texture} and segmentation~\cite{texton1, texton2} and 
taking the form of 
% multidimensional 
histograms on Gabor filter responses. The \emph{bag of words} model~\cite{bow-r, bow-c} is based on the same idea, as a histogram on other visual descriptors. Again, apart from mapping to a new space---that of textons or visual words---they involve local or global spatial pooling.

\emph{Histograms} 
% and every step of building visual features 
can be seen as a form of nonlinear coding followed by pooling~\cite{code-pool}. \emph{Coding} is maybe the most 
important. 
% important factor. 
For example, 
it
% a high-dimensional mapping before pooling, optionally followed by dimension reduction after pooling, 
can reduce interference between elements~\cite{fisher, vlad, emk}. \emph{Weighting} of individual elements is also important in attending 
% important 
regions~\cite{spp, recept-learn, auto-pool} and 
% in 
preventing certain elements from dominating others~\cite{burst, gmp, demo}.

The \emph{pooling operation} itself is any symmetric 
% (permutation-invariant) 
set function of the form $f(X) = g\left(\sum_{x \in X} f(x)\right)$~\cite{deep-sets}, with the most common being average and maximum~\cite{hmax, theor, code-pool}. 

One may pool into
% Apart from a single vector, one may obtain 
\emph{multiple vectors} based on a 
partition in the image~\cite{spp} or feature space~\cite{he, asmk}, 
% spatial partition~\cite{spp} or a partition in the feature space~\cite{he, asmk}, 
but this requires a particular kernel \billc{max or sum operations are also considered kernels?} for matching.

%------------------------------------------------------------------------------

\paragraph{Convolutional networks}

Early
% Following findings of neuroscience, early 
convolutional networks~\cite{neo, lenet} are based on learnable \emph{convolutional layers} interleaved with fixed \emph{spatial pooling layers} that 
downsample.
% downsample, 
% which is an instance of the coding-pooling framework. 
The same design remains until today~\cite{alexnet, vgg, resnet, convnext}. 
Again, apart from mapping to a new space, convolutional layers involve a form of 
local pooling
% weighted local pooling. 
and
% Again, the operation in 
pooling layers 
% is 
commonly 
take
average~\cite{lenet} or maximum~\cite{hmax, alexnet}.

Early networks end in a fully-connected layer over a feature tensor of low resolution~\cite{lenet, alexnet, vgg}. This evolves into spatial pooling, \eg global / regional average followed by a classifier for category-level tasks like classification~\cite{nin, resnet} / detection~\cite{frcnn}, or global maximum followed by a pairwise loss~\cite{mac} for instance-level tasks. 
% This is beneficial for downstream tasks and interpretability~\cite{cam}.

The spatial pooling operation at the end of the network is widely studied in instance level-tasks~\cite{spoc, mac, gem}, giving rise to forms of \emph{spatial attention}~\cite{crow, delf, delg, how, solar}, In category-level tasks, it is more common to study \emph{feature re-weighting} as components of the architecture~\cite{se, cbam, gatherexcite}. The two are closely related because \eg the weighted average is element-wise weighting followed by sum.
% Most modern pooling operations are learnable.

Pooling can be \emph{spatial}~\cite{gatherexcite, delf, delg, how, solar}, \emph{over channels}~\cite{se}, or both \cite{crow, cbam}. CBAM~\cite{cbam} is particularly related to our work in the sense that it includes global average pooling followed by a form of spatial attention, although the latter is not evident in its original formulation and although CBAM is 
not a
% a feature re-weighting rather than 
pooling mechanism.

One
% Apart from a single vector, one 
may obtain \emph{multiple vectors} \eg by some form of clustering~\cite{diffuse} or optimal 
transport~\cite{otk},
% transport~\cite{otk}. 
but this
% This however 
requires a 
% particular 
kernel for matching and is outside the scope of this work. \gkakoc{We have same experiments with k-means and otk. Do you mean only for the kernel, right?}

%------------------------------------------------------------------------------

\paragraph{Vision transformers}

\emph{Pairwise interactions} between features are forms of pooling 
or
% that can be seen as alternatives to convolution or forms of 
\emph{self-attention}
% \emph{self-attention}. 
% Most have been designed as architectural components of convolutional networks, again 
over the spatial~\cite{nln, aa_net, san, n3_net} or channel dimensions~\cite{a2_net, eca}. Originating in language models~\cite{transformer}, \emph{vision transformers}~\cite{vit} streamlined these approaches and 
dominated the architecture \billc{architectural?}landscape.
% became the dominant competitors of convolutional networks. 
Several variants often bring back ideas from convolutional 
networks~\cite{swin, rethinking, levit, cvt, convit, pit, metaformer}.
% networks, including spatial hierarchy~\cite{swin}, relative position encoding~\cite{rethinking, levit}, re-introducing convolution~\cite{cvt, convit}, re-introducing pooling layers~\cite{pit}, or simple pooling instead of attention~\cite{metaformer}.

Transformers downsample only at the input, forming spatial \emph{patch tokens}. Pooling is based on a learnable \cls
% (``classification'') 
token, which, beginning at the input space, undergoes the same self-attention operation with patch tokens and provides a global image representation. That is, the network ends in global weighted average pooling, using as weights the attention of \cls over the patch tokens. 
% Pooling is still gradual, since \cls interacts with patch tokens throughout the network depth.

Few works that have studied 
beyond
% anything other than 
\cls for pooling 
% in transformers 
are mostly limited to global average pooling (GAP)~\cite{swin, rest, halonet, cnnvsvit}. \cls offers attention maps for free,
however
% but those are typically 
of low quality unless in a self-supervised setting~\cite{dino}, which is not well understood. Few works that attempt to rectify this in the supervised setting include a spatial entropy loss~\cite{spatialentropy}, shape distillation from convolutional networks~\cite{intriguing} and skipping computation of self-attention~\cite{skip}.

We attempt to address these limitations and study pooling in convolutional networks, vision transformers, supervised and self-supervised 
% settings 
alike. We derive a simple, attention-based, universal pooling 
mechanism,
% mechanism that applies equally to all cases, 
improving both performance and attention maps.


% \paragraph{Pooling}

% \cite{bilinear, compact-bilinear}
% GAP is proposed in \cite{theor}, gap+max in \cite{gapmax} and an early attention pooling in \cite{gatedatt} -> deep sets.
% BlurPool \cite{blurpool}, i-sqrt cov\cite{isqrtcov}, PSWE \cite{pswe}, Kernel Pooling\cite{kernelpooling}, WELDON \cite{weldon}.

% \paragraph{Vision Transformers}

% MLP spatial mixing instead of attention mixing \cite{resmlp} 
% attention pooling \cite{clip}. 
% \cite{cnnvsvit} here they examine the differences between CNNs and transformers. they say that when trained with GAP, ViTs show less clear localization, but they use JFT-300M for this.
% \cite{refiner} directly refines the attention maps by projecting them to a higher dimensional space to promote their divesity


==> tex/related-4.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Background}

The study of receptive fields~\cite{receptive} lead to the development of 2D \emph{Gabor filters}~\cite{gabor} as a model of the first processing layer in the visual cortex. Visual descriptors based on filter banks in the frequency domain~\cite{gist} and \emph{orientation histograms}~\cite{sift, hog} can be seen as efficient implementations of the same idea. 
% Apart from mapping to a new space---that of filter responses or orientation bins---they involve weighted local spatial pooling.
\emph{Textons}~\cite{texton1, texton2} can be seen as a second layer, taking the form of histograms on Gabor filter responses. The \emph{bag of words} model~\cite{bow-r, bow-c} is based on the same idea, as a histogram on visual descriptors.
% Again, apart from mapping to a new space---that of textons or visual words---they involve local or global spatial pooling.
All these operations involve local or global spatial pooling.

\emph{Histograms} can be seen as a form of nonlinear coding followed by pooling~\cite{code-pool}. \emph{Coding} is maybe the most important. For example, it can reduce interference between elements~\cite{fisher, vlad, emk}. \emph{Weighting} of individual elements is also important in attending regions~\cite{spp, recept-learn, auto-pool} and preventing certain elements from dominating others~\cite{burst, gmp, demo}.
The \emph{pooling operation} itself is any symmetric set function of the form $\pi(X) = g\left(\sum_{x \in X} f(x)\right)$~\cite{deep-sets}, with the most common being average and maximum~\cite{hmax, theor, code-pool}. 

% One may pool into \emph{multiple vectors} based on a partition in the image~\cite{spp} or feature space~\cite{he, asmk}, but this requires a particular kernel \billc{max or sum operations are also considered kernels?} for matching.

%------------------------------------------------------------------------------

\paragraph{Convolutional networks}

Early convolutional networks~\cite{neo, lenet} are based on learnable \emph{convolutional layers} interleaved with fixed \emph{spatial pooling layers} that downsample. The same design remains until today~\cite{alexnet, vgg, resnet, convnext}. Again, apart from mapping to a new space, convolutional layers involve a form of local pooling and pooling layers commonly take average~\cite{lenet} or maximum~\cite{hmax, alexnet}.

Early networks end in a fully-connected layer over a feature tensor of low resolution~\cite{lenet, alexnet, vgg}. This evolves into spatial pooling, \eg global / regional average followed by a classifier for category-level tasks like classification~\cite{nin, resnet} / detection~\cite{frcnn}, or global maximum followed by a pairwise loss~\cite{mac} for instance-level tasks. 

The spatial pooling operation at the end of the network is widely studied in instance level-tasks~\cite{spoc, mac, gem}, giving rise to forms of \emph{spatial attention}~\cite{crow, delf, delg, how, solar}, In category-level tasks, it is more common to study \emph{feature re-weighting} as components of the architecture~\cite{se, cbam, gatherexcite}. The two are closely related because \eg the weighted average is element-wise weighting followed by sum.

Pooling can be \emph{spatial}~\cite{gatherexcite, delf, delg, how, solar}, \emph{over channels}~\cite{se}, or both \cite{crow, cbam}. CBAM~\cite{cbam} is particularly related to our work in the sense that it includes global average pooling followed by a form of spatial attention, although the latter is not evident in its original formulation and although CBAM is 
not a pooling mechanism.

% One may obtain \emph{multiple vectors} \eg by some form of clustering~\cite{diffuse} or optimal transport~\cite{otk}, but this requires a kernel for matching and is outside the scope of this work. \gkakoc{We have same experiments with k-means and otk. Do you mean only for the kernel, right?}

%------------------------------------------------------------------------------

\paragraph{Vision transformers}

\emph{Pairwise interactions} between features are forms of pooling or \emph{self-attention} over the spatial~\cite{nln, aa_net, san, n3_net} or channel dimensions~\cite{a2_net, eca}. Originating in language models~\cite{transformer}, \emph{vision transformers}~\cite{vit} streamlined these approaches and dominated the architecture landscape. Several variants often bring back ideas from convolutional networks~\cite{swin, rethinking, levit, cvt, convit, pit, metaformer}.
\billc{Here we should mention works like \cite{swin, pvt, pvtv2} that perform downsampling inside the transformer; \cite{swin} for classification, \cite{pvt, pvtv2} for detection}

Transformers downsample only at the input, forming spatial \emph{patch tokens}. Pooling is based on a learnable \cls token, which, beginning at the input space, undergoes the same self-attention operation with patch tokens and provides a global image representation. That is, the network ends in global weighted average pooling, using as weights the attention of \cls over the patch tokens. 

Few works that have studied beyond \cls for pooling are mostly limited to global average pooling (GAP)~\cite{swin, rest, halonet, cnnvsvit}. \cls offers attention maps for free, however of low quality unless in a self-supervised setting~\cite{dino}, which is not well studied. Few works that attempt to rectify this in the supervised setting include a spatial entropy loss~\cite{spatialentropy}, shape distillation from convolutional networks~\cite{intriguing} and skipping computation of self-attention~\cite{skip}.
\iavr{or at intermediate layers~\cite{skip}. It has also been found beneficial to inject the \cls token only at the last few layers~\cite{cait}.}
\iavr{there are some works that train transformers with GAP \cite{swin, rest, halonet, cnnvsvit}}
\iavr{in \cite{cnnvsvit} they claim that when trained with GAP, ViTs show less clear localization.}

We attempt to address these limitations and study pooling in convolutional networks, vision transformers, supervised and self-supervised alike. We derive a simple, attention-based, universal pooling mechanism, improving both performance and attention maps.

%------------------------------------------------------------------------------

% \paragraph{Pooling}

% \cite{bilinear, compact-bilinear}
% GAP is proposed in \cite{theor}, gap+max in \cite{gapmax} and an early attention pooling in \cite{gatedatt} -> deep sets.
% BlurPool \cite{blurpool}, i-sqrt cov\cite{isqrtcov}, PSWE \cite{pswe}, Kernel Pooling\cite{kernelpooling}, WELDON \cite{weldon}.

% \paragraph{Vision Transformers}

% MLP spatial mixing instead of attention mixing \cite{resmlp} 
% attention pooling \cite{clip}. 
% \cite{cnnvsvit} here they examine the differences between CNNs and transformers. they say that when trained with GAP, ViTs show less clear localization, but they use JFT-300M for this.
% \cite{refiner} directly refines the attention maps by projecting them to a higher dimensional space to promote their divesity

